Private Adaptive Gradient Methods for Convex Optimization

We study adaptive methods for differentially private convex optimization, proposing and analyzing differentially private variants of a Stochastic Gradient Descent (SGD) algorithm with adaptive stepsizes, as well as the AdaGrad algorithm. We provide upper bounds on the regret of both algorithms and show that the bounds are (worst-case) optimal. As a consequence of our development, we show that our private versions of AdaGrad outperform adaptive SGD, which in turn outperforms traditional SGD in scenarios with non-isotropic gradients where (non-private) Adagrad provably outperforms SGD. The major challenge is that the isotropic noise typically added for privacy dominates the signal in gradient geometry for high-dimensional problems; approaches to this that effectively optimize over lower-dimensional subspaces simply ignore the actual problems that varying gradient geometries introduce. In contrast, we study non-isotropic clipping and noise addition, developing a principled theoretical approach; the consequent procedures also enjoy significantly stronger empirical performance than prior approaches.

==> coord-based-alg.tex <==
\section{Private Adagrad using coordinate-wise projection}
The previous algorithms project the gradient as a vector to some
ellipsoids and can be thought of as dividing the clipping budget
between the different coordinates. In this section, we instead 
clip each coordinate independently to some threshold and divide
the privacy budget between the coordinates.

In particular, at iterate $k$, given samples $\statrv_1,\dots,\statrv_\batch$ with
$g^{k,i} \in \partial F(x^k; \statrv_i)$, we define the following mechanism
for the $j$'th coordinate: first, we project the $j$'th coordinate to 
the range $[-\lambda_j,\lambda_j]$, 
\begin{equation*}
	\tilde g^k_j = \frac{1}{b} \sum_{i=1}^b \pi_{\lambda_j}(g^{k,i}_j),
\end{equation*}
then we add noise to preserve $\diffp_j$-differential privacy,
\begin{equation*}
	\hg^k_j = \tilde g^k_j + \frac{\rho \lambda_j}{\batch \diffp_j} \noise^k_j,  \quad   
			\noise^k_j \simiid \normal(0, 1).
\end{equation*}



We begin by stating the privacy guarantees in the following lemma.
\begin{lemma}
\label{lemma:privacy-coordinate}
	Assume $\sum_{j=1}^d \diffp_j^2 \le \diffp^2$ and
        we run the above iteration for $T \lesssim \frac{n^2}{b^2}$
	iterations. Then the algorithm is $(\rho^2, \diffp^2)$-Renyi differentially 
	private.
\end{lemma}

\begin{proof}[sketch]
	First, the private mechanism of each coordinate 
	preserves $(\rho^2, \diffp_j^2 b^2/n^2)$-Renyi DP. Thus
	the privacy of each iterate is 
	$(\rho^2, \diffp^2 b^2/n^2)$-Renyi DP. Therefore 
	the composition of $T \lesssim n^2/b^2$ iterations
	results in $(\rho^2, \diffp^2)$-Renyi differentially privacy.
\end{proof}


\subsection{Regret bounds for Adagrad}
Let us now analyze the regret bounds that private Adagrad 
achieves using the scheme of the previous section.
For this algorithm, we need the following modification of 
Assumption~\ref{assumption:bounded-moment}.
\begin{assumption} 
\label{assumption:bounded-moment-coord}
For every $1 \le j \le d$ there is $\sigma_j > 0$
such that for any selection $F'(x; \statval) \in \partial F(x;
\statval)$ we have
\begin{equation}  
\label{eqn:moment-matrix-norm}
	\E \left[ | \nabla F_j(x; \statrv) |^p \right ] ^{1/p} \leq \sigma_j,
\end{equation}
where $p \geq 2$ is a positive integer.
\end{assumption}

We have the following bounds in this setting.

\begin{theorem}
  \label{theorem:private-adagrad-coord}
  Let Assumption~\ref{assumption:bounded-moment-coord} hold
  and $x^k$ follow the coordinate-based iteration.
  Let $\diffp_j = \diffp \cdot \frac{\lambda_j^{1/3}}{\sqrt{\sum_{j=1}^d \lambda_j^{2/3}}}$
  and $T = \frac{n^2}{b^2}$.
  Define
  $\wb{x}^T \defeq \frac{1}{T} \sum_{k = 1}^T x^k$. Then
  for any $x\opt \in \xdomain$,
 \begin{align*}
	\E [f(\wb{x}^T) - f(x\opt)]
	& \leq   \frac{\sqrt{2} \diam_\infty(\xdomain)}{T} \sum_{j=1}^d 
		\E \left [ \sqrt{\sum_{k=1}^T (g^{k}_j)^2} \right ] \\ 
		& \quad +  \frac{\sqrt{2} \diam_\infty(\xdomain) \rho 
			     \left( \sum_{j=1}^d \lambda_j^{2/3} \right)^{3/2}}{n \diffp } \\ 
		& \quad + \frac{ \diam_{\infty}(\xdomain)}{(p-1)}
			       \sum_{j=1}^d \frac{\sigma_j^p}{\lambda_j^{p-1}}.
\end{align*}
In particular, setting $\lambda_j = \sigma_j \cdot 
	\left( \frac{n \diffp \sum_{j=1}^d \sigma_j}{( \sum_{j=1}^d \sigma_j^{2/3})^{3/2}} \right)^{1/p}$
yields,
\begin{align*}
	\E [f(\wb{x}^T) - f(x\opt)]
	 & \lesssim  \frac{\diam_\infty(\xdomain)}{T} \sum_{j=1}^d 
		\E \left [ \sqrt{\sum_{k=1}^T (g^{k}_j)^2} \right ] \\ 
		& \quad +  \diam_\infty(\xdomain) \rho 
			      \left(\frac{ \left( \sum_{j=1}^d \sigma_j^{2/3} \right)^{3/2}}
			     {n \diffp } \right)^{1-1/p}
			     \left( \sum_{j=1}^d \sigma_j \right)^{1/p}. 
\end{align*}
\end{theorem}



The proof follows from the next two lemmas which bound 
the bias and second moment.
\begin{lemma}
\label{lemma:private-bias-coord}
Let Assumption~\ref{assumption:bounded-moment-coord} hold. 
Then
\begin{equation*} 
	\bias_1(\tilde g^k) 
		= \E \left[ \lone{\tilde g^k - g^k} \right] 
		\le \sum_{j=1}^d  \frac{\sigma_j^p}{(p-1) \lambda_j^{p-1}}.
		% \frac{\lipobj^p}{(p-1) B_k^{p-1}}.
\end{equation*}
\end{lemma}
\begin{proof}
	Follows immediately from Lemma~\ref{lemma:projection-bias} applied 
	to each coordinate.
\end{proof}



\noindent
The following lemma upper bounds the second moment.
\begin{lemma}
\label{lemma:private-second-moment-coord}
We have that
\begin{equation*} 
	\E \left [ \sum_{j=1}^d \sqrt{\sum_{k=1}^T (\hg^{k}_j)^2} \right ]
		\le \sqrt{2}  \sum_{j=1}^d \E \left [ \sqrt{\sum_{k=1}^T (g^{k}_j)^2} \right ]
			+ \frac{ \sqrt{2} \rho n \left( \sum_{j=1}^d \lambda_j^{2/3} \right)^{3/2}}{\batch^2 \diffp}.
\end{equation*}
\end{lemma}


Theorem~\ref{theorem:private-adagrad-coord} immediately gives the following
corollary for the setting of sub-gaussian coordinates ($ p \ge \log d$).

\begin{corollary}
\label{cor:sub-gaussian-adagrad-coord}
Let Assumption~\ref{assumption:bounded-moment-coord} hold
with $p \ge \log d$. If 
$\batch = 1$, then the coordinate-based Adagrad has
\begin{align*}
\E [f(\wb{x}^T) - f(x\opt)]
	& \lesssim \diam_\infty(\xdomain)  
			 \frac{ \left(\sum_{j=1}^d \sigma_j ^{2/3}\right)^{3/2} }{n \diffp} .
			%\left( \frac{\diam_{\norm{\cdot}_{C^{-1}}}}{\diam_\infty(\xdomain)} \right)^{1/p} .
\end{align*}
\end{corollary}


\subsection{Unknown parameters}
The advantage of the coordinate-base algorithm is that it allows 
an easy (really?) extension to the case when we do not know the
parameters of the distribution. 
In this section, we focus on the setting where 
Assumption~\ref{assumption:bounded-moment-coord} holds
but we do not know the parameters $\sigma_j$. 

The idea is to construct an online estimate $\hat \sigma^k_j$ of the 
true parameters. The following proposition shows that if the online
estimate is accurate on most iterations, then we recover the same
regret bounds.

\begin{theorem}
  \label{theorem:private-adagrad-coord}
  Let Assumption~\ref{assumption:bounded-moment-coord} hold
  and $x^k$ follow the coordinate-based iteration.
  Let $\diffp^k_j = \diffp \cdot \frac{(\lambda^k_j)^{1/3}}{\sqrt{\sum_{j=1}^d (\lambda^k_j)^{2/3}}}$,
  $\lambda^k_j = \hat \sigma^k_j \log d \cdot 
	\left( n \diffp \right)^{1/p}$,
  and $T = \frac{n^2}{b^2}$.
  Define
  $\wb{x}^T \defeq \frac{1}{T} \sum_{k = 1}^T x^k$. 
  If $\hat \sigma^k_j \le \sigma_j / \log d$ for at most $O(\log d)$ iterates,
  and $\hat \sigma^k_j \le \sigma_j \cdot \log d $ for all iterates, then
\begin{align*}
	\E [f(\wb{x}^T) - f(x\opt)]
	& \lesssim  \frac{\diam_\infty(\xdomain)}{T} \sum_{j=1}^d 
		\E \left [ \sqrt{\sum_{k=1}^T (g^{k}_j)^2} \right ] \\ 
		& \quad +  \diam_\infty(\xdomain) \rho
			      \frac{ \left( \sum_{j=1}^d \sigma_j^{2/3} \right)^{3/2}  \log^2 d }
			     {(n \diffp)^{1-1/p} }  \\
		& \quad + \diam_\infty(\xdomain) \frac{\log d ~ \sum_{j=1}^d \sigma_j}{T}.
\end{align*}
\end{theorem}


\begin{proof}
	The proof follows from the next two lemmas and the 
	bounds of Theorem~\ref{theorem:biased-adagrad}:
	Lemma~\ref{lemma:private-bias-coord-unknown} provides 
	an upper bound for the bias and 
	Lemma~\ref{lemma:private-second-moment-coord-unknown}
	provides an upper bound for the second moment.
%	Looking at the bounds of biased Adagrad of Theorem~\ref{theorem:biased-adagrad},
%	the assumption that $\hat \sigma_j \le \sigma_j \cdot \log d $ for all iterates
%	implies the upper bound for the second moment. To bound the bias,
%	note that---as we work with the $\ell_1$-bias---we can bound the bias of 
%	each coordinate separately. For coordinate $j$, the bias can be bounded 
%	by $2 \sigma_j$ at each iteration regardless of $\hat \sigma_j$, therefore
%	for the $O(\log d)$ iterates where $\hat \sigma_j$ is small, we only
%	lose $\sigma_j \log d$ for coordinate $j$. Summing the bias over all 
%	coordinates, we get that the bias (for bad iterates) is bounded by 
%	\begin{align*}
%		\frac{\log d ~ \sum_{j=1}^d \sigma_j}{T}.
%	\end{align*}
\end{proof}



\begin{lemma}
\label{lemma:private-bias-coord-unknown}
Let the conditions of Theorem~\ref{theorem:private-adagrad-coord} hold. 
Then
\begin{equation*} 
	\frac{1}{T} \sum_{k=1}^T \bias_1(\tilde g^k)
		= \frac{1}{T} \sum_{k=1}^T \E \left[ \lone{\tilde g^k - g^k} \right] 
		\le  \frac{ \sum_{j=1}^d \sigma_j}{(p-1) (n \diffp)^{1 - 1/p}} + 
			\frac{\sum_{j=1}^d  \sigma_j \log d}{T}.
\end{equation*}
\end{lemma}
\begin{proof}
	As we want to upper bound the bias for $\lone{\cdot}$, we 
	focus on the $j$'th coordinate.
	Let $S_g = \{k : \hat \sigma^k_j \ge \sigma_j /\log d \}$ be the 
	set of iterates where $\hat \sigma^k_j $ is large 
	and $S_b = [T] \setminus S_g$ be the remaining iterates.
	First, we bound the bias for iterates $k \in S_g$. 
	If $k \in S_g$, then we get that 
	$\lambda_j \ge \sigma_j ~ (n \diffp)^{1/p}$. Therefore 
	for $k \in S_g$ we have using Lemma~\ref{lemma:private-bias-coord}
	that the bias at iteration $k$ is:
	\begin{equation*} 
	\bias(\tilde g^k_j) 
		= \E \left[ |\tilde g^k_j - g^k_j| \right] 
		\le  \frac{\sigma_j^p}{(p-1) (\lambda^k_j)^{p-1}}
		\le  \frac{\sigma_j}{(p-1) (n \diffp)^{1 - 1/p}}.
	\end{equation*}
%	\begin{equation*} 
%	\E \left[ |\tilde g^k_j - g^k_j| \right] 
%		\le  \frac{\sigma_j}{(p-1) (n \diffp)^{1 - 1/p}}.
%	\end{equation*}
	For $k \in S_b$, we have that  
	\begin{equation*} 
	\E \left[ |\tilde g^k_j - g^k_j| \right] 
		\le  \E \left[ |g^k_j| \right] 
		\le \sigma_j,
	\end{equation*}
	where the first inequality follows from the definition of the projection and
	the second inequality follows from Assumption~\ref{assumption:bounded-moment-coord}. 
	Therefore as $| S_b | \le O(\log d)$, we get that 
	\begin{align*} 
	\frac{1}{T} \sum_{k=1}^T \bias(\tilde g^k_j)
		& = \frac{1}{T} \sum_{k \in S_g} \bias(\tilde g^k_j)
			+ \frac{1}{T} \sum_{k \in S_b} \bias(\tilde g^k_j) \\
		& \le \frac{\sigma_j}{(p-1) (n \diffp)^{1 - 1/p}} + 
			\frac{\sigma_j \log d}{T}.
	\end{align*}
	Summing over all coordinates, the claim follows.
\end{proof}



\noindent
The following lemma upper bounds the second moment.
\begin{lemma}
\label{lemma:private-second-moment-coord-unknown}
Let the conditions of Theorem~\ref{theorem:private-adagrad-coord} hold. 
Then
\begin{equation*} 
	\E \left [  \sum_{j=1}^d \sqrt{\sum_{k=1}^T (\hg^{k}_j)^2} \right ]
		\le \sqrt{2}  \sum_{j=1}^d \E \left [ \sqrt{\sum_{k=1}^T (g^{k}_j)^2} \right ]
			+ \sqrt{2} \rho \frac{n \log^2 d \left( \sum_{j=1}^d \sigma_j^{2/3} \right)^{3/2} }
				{\batch^2 \diffp} (n \diffp)^{1/p}.
\end{equation*}
\end{lemma}
\begin{proof}
	The claim follows immediately from Lemma~\ref{lemma:private-second-moment-coord}
	and the assumption that $\hat \sigma^k_j \le \sigma_j \log d$ for all iterates
	which implies that $\lambda^k_j \le  \sigma_j \log^2 d \cdot 
	\left( n \diffp \right)^{1/p}$ for all $k$, hence we get
	\begin{align*}
	{\left( \sum_{j=1}^d \lambda_j^{2/3} \right)^{3/2}}
	\le {\log^2 d \left( \sum_{j=1}^d \sigma_j^{2/3} \right)^{3/2} }(n \diffp)^{1/p}.
	\end{align*}
\end{proof}




\subsubsection{Constructing an online estimate}
\hacomment{How do we get an estimate $\hat \sigma^k_j$
that satisfies our assumptions?}



==> problem_algorithm.tex <==
\section{Problem Formulation \& Algorithm Description}
% In this work, we mainly focus on developing differentially private algorithms for minimizing the empirical loss
% \begin{equation}\label{eqn:emp_loss}
% \min_{x \in  \xdomain} f(x) \defeq \frac{1}{n} \sum_{i=1}^n F(x,z_i),  
% \end{equation}
% where where $ \xdomain$ is a convex subspace of $\R^d$ and $F(x,z)$ is the loss of model $x$ over data point $z \in \mathcal{Z}$. Also, recall that $\mathcal{S} = (z_1,...,z_n) \in \mathcal{Z}^n$ denotes the dataset.
% This is mainly motivated by the the problem of minimizing the population loss 
% \begin{equation}\label{eqn:main-prob}
% \E[F(x; \statrv)]
%  = \int F(x; \statval) dP(\statval),
% \end{equation}
% and here we assume $z_i$'s are drawn independently from distribution $P$.



% Both algorithms run in iterations. At iteration $k$, we take a batch $\mathcal{D}_k:= \{z_i^k\}_{i=1}^b$ with size $b$, and compute subgradients
% $g^{k,i} \in \partial F(x^k; z_i^k)$ where $x^k$ is the $k$-th iterate. Next, we consider an ellipsoid $E_{A_k}$ for some $A_k \succ 0_{d \times d}$, and project each subgradient to it, and then take an average, i.e.,
% \begin{equation*}
% \tilde g^k = \frac{1}{\batch} \sum_{i=1}^\batch \pi_{A_k}(g^{k,i}),
% \end{equation*}
% We then define $\hg_k$, the privatized version of $\tilde g^k $, to be
% \begin{equation*}
%  \hg^k = \tilde g^k + \frac{\rho}{\batch \diffp} \noise^k,  \quad   \noise^k \simiid \normal(0, A_k^{-1}).
% \end{equation*}
% Finally, using the privatized gradient $\hg_k$, we can now use 
% SGD or Adagrad updates yielding the following private SGD update:
% \begin{equation}
% \label{eqn:private-sgd}
% x^{k+1} =  \proj_{\xdomain}( x^k -  \alpha_k \hg^k),
% \end{equation}
% and the following private Adagrad:
% \begin{equation}
% \label{eqn:private-adagrad}
% x^{k+1} =  \proj_{\xdomain}( x^k -  H_k^{-1}  \hg^k),
% \end{equation}
% where $H_k = \frac{1}{\alpha} \diag\left(\sum_{i=1}^{k} \hg^i \hg^{i^T}  \right)^{\frac{1}{2}}$.
